Shipwright: A Human-in-the-Loop System for Dockerfile Repair

Docker is a tool for lightweight OS-level virtualization. Docker images are created by performing a build, controlled by a source-level artifact called a Dockerfile. We studied Dockerfiles on GitHub, and -- to our great surprise -- found that over a quarter of the examined Dockerfiles failed to build (and thus to produce images). To address this problem, we propose SHIPWRIGHT, a human-in-the-loop system for finding repairs to broken Dockerfiles. SHIPWRIGHT uses a modified version of the BERT language model to embed build logs and to cluster broken Dockerfiles. Using these clusters and a search-based procedure, we were able to design 13 rules for making automated repairs to Dockerfiles. With the aid of SHIPWRIGHT, we submitted 45 pull requests (with a 42.2% acceptance rate) to GitHub projects with broken Dockerfiles. Furthermore, in a "time-travel" analysis of broken Dockerfiles that were later fixed, we found that SHIPWRIGHT proposed repairs that were equivalent to human-authored patches in 22.77% of the cases we studied. Finally, we compared our work with recent, state-of-the-art, static Dockerfile analyses, and found that, while static tools detected possible build-failure-inducing issues in 20.6--33.8% of the files we examined, SHIPWRIGHT was able to detect possible issues in 73.25% of the files and, additionally, provide automated repairs for 18.9% of the files.

==> Makefile <==
NAME:=main

# To update, run: latex-process-inputs -makefilelist main.tex
TEX_FILES = \
$(NAME).tex

PDFS := paper.pdf
TEMP_TXTS := $(patsubst %.pdf,%.txt,$(PDFS))
OUTPUTS_SPELL := $(TEMP_TXTS)

.DEFAULT_GOAL := pdf

pdf:
#	latexmk -bibtex -pdf $(NAME)
	latexmk -pdf $(NAME)

final: pdf
	@echo '******** Did you spell-check the paper? ********'
	pdffonts $(NAME).pdf; fi

clean:
	-rm -f *aux *bbl *blg *log *.dvi $(NAME).pdf *.fdb_latexmk *.fls *.out *.spl

check: $(TEMP_TXTS)
	cat $^ | aspell list --extra-dicts=./okwords.en.pws | sort | uniq

%.txt: paper.pdf
	pdftotext $<

%.err: %.txt
	cat $^ | aspell list --extra-dicts=./okwords.en.pws | sort | uniq

.PHONY: all

tags: TAGS
TAGS: ${TEX_FILES}
	etags ${TEX_FILES}


==> figs/cluster-results-table.tex <==

\begin{table}[t]
\caption{
Usage of recommendations and repairs to address broken Dockerfiles within each cluster.
}
\label{table:cluster-results}
\centering
% \resizebox{\columnwidth}{!}
% {
\begin{tabular}{ccccc}
\toprule
% First two column labels
\multicolumn{2}{c}{Cluster Stats.} & \multicolumn{3}{c}{\tname{}} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-5} Index & Files &  Coverage & \# Recom. & \# Repair \\ 
\midrule
% MAIN TABLE STARTS HERE
\csvreader[
head to column names,
late after line=\\,
late after last line=\\\midrule
]{data/cluster-results-table.csv}{}%
{
  \clusterIndex & 
  \clusterFiles &
  \coverage & 
  \recommendations & 
  \repairs 
}%
\end{tabular}
% }
\end{table}
